Classical and learned MR to pseudo-CT mappings for accurate transcranial ultrasound simulation

Model-based treatment planning for transcranial ultrasound therapy typically involves mapping the acoustic properties of the skull from an x-ray computed tomography (CT) image of the head. Here, three methods for generating pseudo-CT images from magnetic resonance (MR) images were compared as an alternative to CT. A convolutional neural network (U-Net) was trained on paired MR-CT images to generate pseudo-CT images from either T1-weighted or zero-echo time (ZTE) MR images (denoted tCT and zCT, respectively). A direct mapping from ZTE to pseudo-CT was also implemented (denoted cCT). When comparing the pseudo-CT and ground truth CT images for the test set, the mean absolute error was 133, 83, and 145 Hounsfield units (HU) across the whole head, and 398, 222, and 336 HU within the skull for the tCT, zCT, and cCT images, respectively. Ultrasound simulations were also performed using the generated pseudo-CT images and compared to simulations based on CT. An annular array transducer was used targeting the visual or motor cortex. The mean differences in the simulated focal pressure, focal position, and focal volume were 9.9%, 1.5 mm, and 15.1% for simulations based on the tCT images, 5.7%, 0.6 mm, and 5.7% for the zCT, and 6.7%, 0.9 mm, and 12.1% for the cCT. The improved results for images mapped from ZTE highlight the advantage of using imaging sequences which improve contrast of the skull bone. Overall, these results demonstrate that acoustic simulations based on MR images can give comparable accuracy to those based on CT.

==> figs/fig1/input_example.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=1.318in,
height=1.343in,
at={(0.512in,2.299in)},
scale only axis,
axis on top,
xmin=0.5,
xmax=256.5,
y dir=reverse,
ymin=-1.98752714494421,
ymax=258.987527144944,
axis line style={draw=none},
ticks=none,
title style={font=\bfseries},
title={ZTE}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=256.5, ymin=0.5, ymax=256.5] {figs/fig1/input_example-1.png};
\end{axis}

\begin{axis}[%
width=1.273in,
height=1.298in,
at={(2.249in,2.299in)},
scale only axis,
axis on top,
xmin=0.5,
xmax=256.5,
y dir=reverse,
ymin=-1.98752714494421,
ymax=258.987527144944,
axis line style={draw=none},
ticks=none,
title style={font=\bfseries},
title={T1}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=256.5, ymin=0.5, ymax=256.5] {figs/fig1/input_example-2.png};
\end{axis}

\begin{axis}[%
width=1.272in,
height=1.297in,
at={(0.516in,0.433in)},
scale only axis,
axis on top,
xmin=0.5,
xmax=256.5,
y dir=reverse,
ymin=-1.98752714494412,
ymax=258.987527144944,
axis line style={draw=none},
ticks=none,
title style={font=\bfseries},
title={Mask}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=256.5, ymin=0.5, ymax=256.5] {figs/fig1/input_example-3.png};
\end{axis}

\begin{axis}[%
width=1.272in,
height=1.297in,
at={(2.252in,0.433in)},
scale only axis,
axis on top,
xmin=0.5,
xmax=256.5,
y dir=reverse,
ymin=-1.98752714494412,
ymax=258.987527144944,
axis line style={draw=none},
ticks=none,
title style={font=\bfseries},
title={Ground truth CT}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=256.5, ymin=0.5, ymax=256.5] {figs/fig1/input_example-4.png};
\end{axis}
\end{tikzpicture}%
